CFLOBDDs: Context-Free-Language Ordered Binary Decision Diagrams

This paper presents a new compressed representation of Boolean functions, called CFLOBDDs (for Context-Free-Language Ordered Binary Decision Diagrams). They are essentially a plug-compatible alternative to BDDs (Binary Decision Diagrams), and hence useful for representing certain classes of functions, matrices, graphs, relations, etc. in a highly compressed fashion. CFLOBDDs share many of the good properties of BDDs, but--in the best case--the CFLOBDD for a Boolean function can be exponentially smaller than any BDD for that function. Compared with the size of the decision tree for a function, a CFLOBDD--again, in the best case--can give a double-exponential reduction in size. They have the potential to permit applications to (i) execute much faster, and (ii) handle much larger problem instances than has been possible heretofore. CFLOBDDs are a new kind of decision diagram that go beyond BDDs (and their many relatives). The key insight is a new way to reuse sub-decision-diagrams: components of CFLOBDDs are structured hierarchically, so that sub-decision-diagrams can be treated as standalone ''procedures'' and reused. We applied CFLOBDDs to the problem of simulating quantum circuits, and found that for several standard problems the improvement in scalability--compared to simulation using BDDs--is quite dramatic. In particular, the number of qubits that could be handled using CFLOBDDs was larger, compared to BDDs, by a factor of 128x for GHZ; 1,024x for BV; 8,192x for DJ; and 128x for Grover's algorithm. (With a 15-minute timeout, the number of qubits that CFLOBDDs can handle are 65,536 for GHZ, 524,288 for BV; 4,194,304 for DJ; and 4,096 for Grover's Algorithm.)

==> back.tex <==
% -*- TeX-master: t; TeX-PDF-mode: t -*-

\section{Background}
\label{Se:Background}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> limitations.tex <==
% -*- TeX-master: t; TeX-PDF-mode: t -*-

\section{Limitations of CFLOBDDs}
\label{Se:Limitations}

\twr{UNDER CONSTRUCTION}

\twrnew{
In this section, we discuss how some known limitations of BDDs still hold for CFLOBDDs.
In particular, a CFLOBDD representation of multiplication is still inherently exponential because the middle vertices of the outermost grouping represent the same functions as the half-height vertices of the BDD for multiplication that uses the same variable order.
[CHECK that the inherent bound on multiplication with BDDs gives a lower bound on the number of half-height vertices.]
}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

==> notes.tex <==
Shortlist
=========
[DONE] Hash-consing vs. canonicity

[DONE] In the discussion of canonicity, change ``identical,'' ``structurally equal,'' and ``='' to isomorphic

[DONE] Example for ApplyAndReduce (Fig. 5 doesn't work because it does not trigger any propagation)

Rationale for the structural invariants

Limitations
 o multiplication, representing QFT matrix (?)
 o Bound on CFLOBDD size from converting a BDD to a CFLOBDD

Finish quantum experiments with the two tensor-network packages

Re-run experiments on a single OS

Add appendices about two new kinds of quantum gates

Revise discussion of QFT

Related Work

Move longer tables from Appendices into the Evaluation section

---------------------------------------------

What is the reason for each of these pieces of terminology?
What is their semantics?
More generally, what are the requirements of the data structure, and how do the various components of CFLOBDDs fulfill those requirements?

 CFLOBDDs are a plug-compatible replacement for BDDs.
 That is, given a client algorithm that uses BDDs as their underlying data structure with an interface to the data structure’s operations, we can, in principle, replace the BDD library with a CFLOBDD library without changing anything on the client side.
 CFLOBDD operations are one-for-one with BDD operations, although the internals are different.
 In some cases, such as matrix-manipulation algorithms (and Quantum Fourier Transform), the BDD operation is based on a divide-by-2 divide-and-conquer algorithm whereas the corresponding CFLOBDD operation is a $\sqrt{N}$-by-$\sqrt{N}$ divide-and-conquer algorithm.
 However, such details would be hidden from the client by the library interface.
 

=========================================




==> overview-old.tex <==
% -*- TeX-master: t; TeX-PDF-mode: t -*-

\section{Overview}
\label{Se:Overview}

\begin{figure}
    \centering
    $\begin{array}{c@{\hspace{6ex}}c}
      H_2 ~~ = ~~
        \kbordermatrix{
            & 0 & 1\\
          0 & 1 & 1\\
          1 & 1 & -1\\
        }
      &
      H_4 = H_2 \tensor H_2
          = \begin{bmatrix}
              H_2 & H_2\\
              H_2 & -H_2\\
              \end{bmatrix}
         ~~ = ~~
         \kbordermatrix{
              & 00 & 01 & 10 & 11\\
           00 & 1 & 1 & 1 & 1\\
           01 & 1 & -1 & 1 & -1\\
           10 & 1 & 1 & -1 & -1\\
           11 & 1 & -1 & -1 & 1\\
         }
    \end{array}$
    \caption{$H_2$ and $H_4$, the first two members of the family of Hadamard matrices $\HadamardFamily = \{ H_{2^i} \mid i \geq 1 \}$.}
    \label{Fi:HadamardMatrices}
\end{figure}

This section describes the principles behind CFLOBDDs, and compares them with BDDs.
We use as an example a family of Hadamard matrices $\HadamardFamily = \{ H_{2^i} \mid i \geq 1 \}$, which will play a role later in \sectrefsp{efficient-relations}{quantum-algos}{evaluation}.
\figref{HadamardMatrices} shows $H_2$ and $H_4$, the first two matrices in $\HadamardFamily$.
The Hadamard matrices can be defined recursively:
for $i \geq 1$, $H_{2^{i+1}} = H_{2^i} \tensor H_{2^i}$,
with $H_2$ from \figref{HadamardMatrices} as the base case.
where $\tensor$ denotes Kronecker product.\footnote{
  \label{Footnote:KroneckerProduct}
  Others use a different indexing scheme:
  $H_2$ is the same as with our scheme (as is $H_4$), but the recursive definition is $H_{2^{i+1}} = H_2 \tensor H_{2^i}$, for $i \geq 1$.
  Thus, for $i \geq 0$, $H_{2^i}$ is a $2^i \times 2^i$ matrix (and thus has $2^{2i}$ entries).
  In contrast, with our indexing scheme, the matrix we call $H_{2^i}$ is a $2^{2^{i-1}} \times 2^{2^{i-1}}$ matrix, for $i \geq 1$ (and thus has $2^{2^i}$ entries).

  \hspace{1.5ex}
  Put another way, what we call $H_{2^i}$ would conventionally be known as $H_{2^{2^{i-1}}}$.
  Not only do we avoid having to write a doubly superscripted subscript, we will see in \sectref{ReuseOfGroupings} that the recursive rule ``$H_{2^{i+1}} = H_{2^i} \tensor H_{2^i}$'' fits particularly well with the internal structure of CFLOBDDs.
}
The \emph{Kronecker product} of two matrices is defined as follows:
\begin{equation*}
  A \tensor B = \left[ \begin{array}{ccc}
                              a_{1,1} & \cdots & a_{1,m} \\
                              \vdots  & \ddots & \vdots  \\
                               a_{n,1} & \cdots & a_{n,m}
                             \end{array}
                    \right] \otimes B
              = \left[ \begin{array}{ccc}
                              a_{1,1}B & \cdots & a_{1,m}B \\
                               \vdots  & \ddots & \vdots   \\
                              a_{n,1}B & \cdots & a_{n,m}B
                             \end{array}
                    \right]
\end{equation*}
Equivalently, $(A \tensor B)_{ii',jj'} = A_{i,j} \times B_{i',j'}$.
If $A$ is $n \times m$ and $B$ is $n' \times m'$, then $A \otimes B$ is $nn' \times mm'$.
\Omit{It is easy to see that the Kronecker product is associative, i.e.,
\begin{center}
  $(A \otimes B) \otimes C = A \otimes (B \otimes C)$.
\end{center}
}
Thus, the number of rows/columns/entries in $H_{2^{i+1}}$ is the \emph{square} of the number of rows/columns/entries in $H_{2^i}$.
For example, $H_4$ is $4 \times 4$ (16 entries);
$H_8$ is $16 \times 16$ (256 entries).

For $i \geq 1$, $H_{2^i}$ is a square matrix of size $2^{2^{i-1}} \times 2^{2^{i-1}}$.
Thus, an indexing scheme for $H_{2^i}$ can be defined that uses $2^{i-1} + 2^{i-1}$ $= 2 * 2^{i-1}$ $= 2^i$ Boolean variables.
As shown in \figref{HadamardMatrices}, $H_2$ requires 2 variables and $H_4$ requires 4 variables.
In general, $H_{2^i}$ can be treated as a Boolean function of type $\{0,1\}^{2^{i-1}}\times \{ 0,1 \}^{2^{i-1}} \rightarrow \{-1, 1\}$.
If $H_{2^i}$ were represented as a decision tree (of height $2^{i}$),
it would have $2^{2^{i}}$ leaves and $2^{2^{i}} - 1$ internal nodes, and thus the size of the representation is doubly exponential in $i$.
As we will see, there is a BDD encoding of $H_{2^i}$ of size $O(2^i)$, and hence BDDs achieve exponential compression on $\HadamardFamily$, compared to the decision tree.
In contrast, there is a CFLOBDD encoding of $H_{2^i}$ of size $O(i)$, and thus CFLOBDDs achieve \emph{double-exponential} compression on $\HadamardFamily$.
Moreover, in \sectref{Separation:HadamardRelation}, we show that this exponential separation is inherent:
a BDD that represents $H_{2^i}$ requires $\Omega(2^i)$ nodes (\theoref{HadamardSeparation}).

\begin{figure}[tb!]
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.5]{figures/walsh1_dd.pdf}
    \caption{Decision tree}
    \label{Fi:walsh1_dd}
    \vspace{4ex}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.5]{figures/walsh1_bdd_new.pdf}
    \caption{BDD}
    \label{Fi:walsh1_bdd}
    \vspace{4ex}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.45]{figures/walsh1_label-cropped.pdf}
    \caption{CFLOBDD}
    \label{Fi:walsh1_label}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[scale=0.5]{figures/walsh1_label_pathFT.pdf}
    \caption{The path for assignment $[{x_0} \mapsto F, {y_0} \mapsto T]$ in (c)
    }
    \label{Fi:walsh1_path}
    \end{subfigure}
    \caption{
    Three representations of $H_2$, all using the variable ordering $\langle x_0, y_0 \rangle$:
    (a) as a decision tree, (b) as a BDD, and (c) as a CFLOBDD.
    In (a), (b), and (d), the \textbf{bold} arrows and arcs highlight the path for the assignment $[{x_0} \mapsto F, {y_0} \mapsto T]$.
    }
    \label{Fi:walsh1}
\end{figure}

\subsection{Encoding $H_2$: Decision Trees and BDDs}

\figref{walsh1_dd} shows the decision tree for $H_2$, which has $2$ plies, $3$ interior nodes, and $4$ leaf nodes.
It uses the variable ordering $\langle x_0, y_0 \rangle$, associating $x_0$ to the first ply and $y_0$ to the second ply.
$x_0$ and $y_0$ represent the row and column variables of $H_2$, respectively.
At each interior node, the left branch is followed when the current Boolean variable in an assignment has the value $F$ (or $0$);
the right branch is followed for the value $T$ (or $1$).
The $[0,1]$ entry of $H_2$, has the value $1$.
In the decision tree, $H_2[0,1]$ corresponds to the path for the assignment $[{x_0} \mapsto F, {y_0} \mapsto T]$, which is highlighted in bold in \figref{walsh1_dd}.

The BDD for $H_2$, also using the variable ordering $\langle x_0, y_0 \rangle$, is shown in~\figref{walsh1_bdd}.
Again, left branches are for $F$; right branches are for $T$.
In $H_2$, rows $0$ and $1$ are different, and hence the BDD node for $x_0$ is a $\textit{fork\_node}$, which forks to two different substructures.
In row $0$ of the matrix, columns $0$ and $1$ are identical, and hence the BDD node for $y_0$ in the $F$ branch of $x_0$ is skipped with the $F$ branch of $x_0$ leading directly to the terminal value.
Conversely, for row $1$ of $H_2$ the columns differ, and hence the BDD node for $y_0$ in the $T$ branch of $x_0$ is a $\textrm{fork\_node}$.
The total number of nodes in the BDD representation is four.
In the BDD, $H_2[0,1]$ again corresponds to the path for the assignment $[{x_0} \mapsto F, {y_0} \mapsto T]$, which is highlighted in bold in \figref{walsh1_bdd}.
(Only the edge for $x_0 \mapsto F$ is highlighted because the ply for $y_0$ is skipped when $x_0 \mapsto F$.)

\subsection{Encoding $H_2$ with a CFLOBDD}

% CFLOBDDs can be considered to be a variant of BDDs in which further folding is performed on the graph.
The CFLOBDD representation of $H_2$ consists of three \emph{groupings}, shown as three ovals in \figref{walsh1_label}.\footnote{
  \label{Footnote:NodeGroupingVertexTerminology}
  Groupings are represented in memory as a kind of node structure, but we will use ``nodes'' solely for BDD nodes.
  Groupings are depicted as ovals, and the dots inside will be referred to as ``vertices.''
}
Each CFLOBDD grouping is associated with a given \emph{level}.
The two small ovals are at level $0$ (labeled $L_0$), and the large oval is at level $1$ (labeled $L_1$).
There is an implicit hierarchical structure to the levels, and level-$0$ groupings are said to be \emph{leaves} of the CFLOBDD.
There are only two possible types of level-0 groupings:
\begin{itemize}
  \item
    A level-0 grouping like the one at the upper right in \figref{walsh1_label} is called a \emph{fork grouping}.
  \item
    A level-0 grouping like the one at the lower right in \figref{walsh1_label} is called a \emph{don't-care grouping}.
\end{itemize}
The vertex at the top of each grouping is the grouping's \emph{entry vertex}.
In all cases, the entry vertex of a level-$0$ grouping corresponds to a decision point (or ``node'') in the corresponding decision tree.

In matrix $H_2$, each entry is either $1$ or $-1$.
When encoded correctly as a CFLOBDD, each assignment to the Boolean variables $x_0$ and $y_0$ corresponds to a path in the CFLOBDD that leads to either $1$ or $-1$, as appropriate.
Each such path starts from the entry vertex of the highest-level grouping (i.e., in \figref{walsh1_label}, the entry vertex of the level-$1$ grouping), making ``decisions'' for the next variable in sequence each time the entry vertex of a level-$0$ grouping is encountered.

\figref{walsh1_path} illustrates the key principle behind CFLOBDDs---namely, how a \emph{matched-path} condition on paths allows a given region of a graph to play multiple roles during the evaluation of a Boolean function.
The assignment $[{x_0} \mapsto F, {y_0} \mapsto T]$ corresponds to the matrix entry $H_2[0,1]$, which has the value $1$.
The path for $[{x_0} \mapsto F, {y_0} \mapsto T]$ is shown in bold in the CFLOBDD structure in \figref{walsh1_path}.
The path starts at the level-$1$ grouping's entry vertex and goes
to the entry vertex of the level-$0$ fork grouping via a solid edge (---);
takes the left branch of the fork grouping (corresponding to $x_0 \mapsto F$);
and leaves the fork grouping via a solid edge (---), reaching the leftmost of the vertices in the middle of the level-$1$ grouping.
The second part of the path continues to the entry vertex of the level-$0$ don't-care grouping via a dashed-dotted edge ($-\cdot\cdot\,-$);
takes the right branch of the don't-care grouping (corresponding to $y_0 \mapsto T$);
and leaves via a dashed-dotted edge ($-\cdot\cdot\,-$), reaching the leftmost exit vertex of the level-$1$ grouping, which is connected to the terminal value $1$ (as expected).
A pair of incoming and outgoing edges of a grouping, such as the pairs of solid edges and dashed-dotted edges traversed by the bold path in \figref{walsh1_path}, are said to be \emph{matched}.
The bold path itself is called a \emph{matched path}.\footnote{
    \label{Fo:MatchedPathExplanation}
    Solid, dotted, dashed and dashed-dotted edges are used in the figures shown here rather than attaching explicit labels to them.
    Formally, the matched-path principle can be expressed as a condition
    that---for a path to be \emph{matched}---the word spelled out by the labels on the edges of the path must be a word in a certain context-free language, as described below.
    (This idea is the origin of ``CFL'' in ``CFLOBDD''.)

    \hspace{1.5ex}
    One way to formalize the condition is to label each edge from level $i$ to level $i-1$ with an open-parenthesis symbol of the form ``$(_b$'', where $b$ is an index that distinguishes the edge from all other edges to any entry vertex of any grouping of the CFLOBDD.
    (In particular, suppose that there are  $\NumConnections$ such edges, and that the value of $b$ runs from $1$ to $\NumConnections$.)
    Each return edge that runs from an exit vertex of the level $i-1$ grouping back to level $i$, and corresponds to the edge labeled ``$(_b$'', is labeled ``$)_b$''.

    \hspace{1.5ex}
    Each path in a CFLOBDD then generates a string of parenthesis symbols formed by concatenating, in order, the labels of the edges on the path.
    (Unlabeled edges in the level-$0$ groupings are ignored in forming this string.)
    A path in a CFLOBDD is called a \emph{$\Matched$-path} iff the path's word is in the language $L(\Matched)$ of balanced-parenthesis strings generated from  non-terminal $\Matched$ according to the following context-free grammar:
    \begin{center}
    \begin{tabular}{@{\hspace{0in}}r@{\hspace{.05in}}c@{\hspace{.05in}}l@{\hspace{.1in}}r@{\hspace{0in}}}
      $\Matched$ & $\rightarrow$ & $\Matched~\Matched$ & \\
                 & $|$           & ${(_b}~\Matched~{)_b}$ & $1 \leq b \leq \NumConnections$ \\
                 & $|$ & $\epsilon$ &
    \end{tabular}
    \end{center}
    Only $\Matched$-paths that start at the entry vertex of the CFLOBDD's highest-level grouping and end at one of the final values are considered in interpreting CFLOBDDs.
  }

This example illustrates the following principle:

\begin{mdframed}[innerleftmargin = 3pt, innerrightmargin = 3pt, skipbelow=-0.0em]
  $\MPP$.  {\em When a path follows an edge that returns to level $i$ from level $i-1$, it must follow an edge that matches the closest preceding edge from level $i$ to level $i-1$.\/}
\end{mdframed}

The matched-path principle allows a given grouping of a CFLOBDD to do double duty (and, in general, to perform multiple roles).
For example, the level-$0$ fork grouping in~\figref{walsh1_label} is used to interpret
(i) $x_0$ (when ``called'' via the solid edge), and
(ii) $y_0$ (when ``called'' via the dashed edge, which happens when
$x_0 \mapsto T$).
The edge-matching condition is important because the solid return edges lead to the level-$1$ grouping's middle vertices, whereas the dashed return edges lead to the level-$1$ grouping's exit vertices.

In \figref{walsh1}(c), the fork grouping is labeled with $x_0$ and $y_0$, and the don't-care grouping is labeled with only $y_0$.
As discussed in the previous paragraph, level-$0$ groupings are shared, and thus are used to interpret \emph{different variables at different places in a matched path through a CFLOBDD}.
For that reason, in later diagrams the level-$0$ groupings are not labeled with specific variables.

At this point, it is useful to introduce some terminology to refer to the individual components of CFLOBDDs and groupings within CFLOBDDs.
\begin{itemize}
  \item
    The collection of vertices positioned at the middle of each grouping at level $1$ or higher is called the grouping's \emph{middle vertices}.
    We assume that a grouping's middle vertices are arranged in some fixed known order (e.g., they can be stored in an array).
  \item
    The collection of vertices positioned at the bottom of each grouping is called the grouping's \emph{exit vertices}.
    We assume that a grouping's exit vertices are arranged in some fixed known order (e.g., they can be stored in an array).
  \item
    The edge that emanates from the entry vertex of a level-$i$ grouping $g$ and leads to a level $i-1$ grouping is called $g$'s \emph{$A$-connection}.
  \item
    An edge that emanates from a middle vertex of a level-$i$ grouping $g$ and leads to a level $i-1$ grouping is called a \emph{$B$-connection} of $g$.
  \item
    The edges that emanate from the exit vertices of a level $i-1$ grouping and lead back to a level $i$ grouping are called \emph{return edges}.
  \item
    The edges that emanate from the exit vertices of the highest-level grouping and lead to a terminal value are called \emph{value edges}.
    In the case of a Boolean-valued CFLOBDD, the highest-level grouping has at most two exit vertices, and these are mapped uniquely to $\{F,T\}$.
    In the case of a multi-terminal CFLOBDD, there can be an arbitrary number of exit vertices, which are mapped uniquely to values drawn from some finite set.
    (\figref{walsh1_label} is a multi-terminal CFLOBDD;
    the level-$1$ grouping has two exit vertices that are mapped to $1$ and $-1$.)
\end{itemize}

In \figref{walsh1_label}, the grouping at level $1$ in some sense encompasses both variables $x_0$ and $y_0$ via a mechanism that can be thought of as a procedure call that has multiple return points.
In \figref{walsh1_label}, the $A$-connection in the level-$1$ grouping calls the fork grouping, whose two exit vertices
respectively return to the two middle vertices in the level-$1$ grouping.
(Variable $x_0$ is interpreted in this call.)
The $B$-connection from the leftmost middle vertex calls the don't-care grouping, whose one exit vertex returns to the leftmost level-$1$ exit vertex, which is associated with the terminal value $1$.
The $B$-connection from the rightmost middle vertex calls the fork grouping, whose two exit vertices respectively return to the two level-$1$ exit vertices
(Variable $y_0$ is interpreted in the calls to the B-connection groupings).
In \figref{walsh1_label}, matching calls and returns are shown either as a pair of solid edges, dashed edges, or dashed-dotted edges.

As illustrated above, CFLOBDDs can be considered to be a variant of BDDs in which further folding is performed on the graph.
One might be worried by such a concept, because BDDs are DAGs, and some foldings of a DAG lead to \emph{cyclic} graphs---and hence an \emph{infinite} number of paths.
For instance, if one ignores the ovals in \figref{walsh1_label}, as well as the distinction between solid and dashed edges, one is left with a cyclic graph:
there is a cycle that starts at the rightmost middle vertex of the level-$1$ grouping, follows the dashed edge ($\text{-}\,\text{-}\,\text{-}$) to the entry vertex of the level-$0$ fork-grouping, takes the right branch, and returns along the solid edge (---) to the rightmost middle vertex of the level-$1$ grouping.
However, that path is excluded from consideration because it is not a matched path:
the solid edge does not match with the preceding dashed edge.

In essence, a CFLOBDD is a kind of non-recursive hierarchical finite-state machine (HFSM) \cite{DBLP:journals/toplas/AlurBEGRY05}, whereas an OBDD is (essentially) an acyclic ordinary FSM.
Moreover, a CFLOBDD is an HFSM of a particularly restricted kind.
\twr{TODO: Say where the restrictions are stated.}
One consequence is that every matched path through a CFLOBDD starting from the entry vertex of the outermost grouping (at level $k$) is of the same length;
each such path reaches the entry vertex of a level-$0$ grouping the same number of times, namely, $2^k$, and ends at some terminal value $v \in V$, where $V$ is some domain of values.
Consequently, each (multi-terminal) CFLOBDD represents a Boolean function of the form $\{ T,F \}^{2^k} \rightarrow V$.


\subsection{Representing Multi-Terminal CFLOBDDs}
\label{Se:PseudoCodeDefinitions}

\begin{figure}[tb!]
%\removelatexerror
{
\LinesNotNumbered
\setlength{\interspacetitleruled}{0pt}%
\setlength{\algotitleheightrule}{0pt}%
{\small
\begin{algorithm*}[H]
\DontPrintSemicolon
%\caption{Specifications of Grouping, InternalGrouping, DontCareGrouping, ForkGrouping, CFLOBDD\label{Fi:ClassDefinitions}}
abstract class Grouping \{\;
\Indp    
    level: int\;
    numberOfExits: int\;
\Indm \}\;
class InternalGrouping extends Grouping \{\;
\Indp
    AConnection: Grouping\;
    AReturnTuple: ReturnTuple\;
    numberOfBConnections: int\;
    BConnections: array[1..numberOfBConnections] of Grouping\;
    BReturnTuples: array[1..numberOfBConnections] of ReturnTuple\;
\Indm \}\;
class DontCareGrouping extends Grouping \{\;
\Indp
    level = 0\;
    numberOfExits = 1\;
\Indm \}\;
class ForkGrouping extends Grouping \{\;
\Indp
    level = 0\;
    numberOfExits = 2\;
\Indm \}\;
class CFLOBDD \{\qquad  \tcp{Multi-terminal CFLOBDD}
\Indp
    grouping: Grouping\;
    valueTuple: ValueTuple\;
\Indm\}\;
\end{algorithm*}
}
}
\caption{Datatypes for Grouping, InternalGrouping, DontCareGrouping, ForkGrouping, and CFLOBDD\label{Fi:ClassDefinitions}.}
\end{figure}

\begin{figure}[tb!]
    \centering
    \includegraphics[scale=0.45]{figures/walsh1-rep-cropped.pdf}
    \caption{The CFLOBDD from \figref{walsh1_label} depicted as an instance of the class {\tt CFLOBDD\/} defined in ~\figref{ClassDefinitions}.}
    \label{Fi:product4Figure}
\end{figure}

As is apparent from \figref{walsh1_label}, there is a good deal of structure inside a CFLOBDD grouping---whereas a BDD node has no internal structure (beyond the two pointers to its two children).
We will use an object-oriented pseudo-code to define the classes that are used for representing multi-terminal CFLOBDDs, and various operations on objects in these classes.
The basic classes are defined in ~\figref{ClassDefinitions}: {\tt Grouping}, {\tt InternalGrouping}, {\tt DontCareGrouping}, {\tt ForkGrouping}, and {\tt CFLOBDD}.
\figref{product4Figure} shows how the CFLOBDD from \figref{walsh1_label} is represented as an instance of class {\tt CFLOBDD}.
More details about the notation used in our pseudo-code notation to manipulate CFLOBDDs and their components can be found in Appendix~\sectref{additional-notation}.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.47\linewidth}
    \includegraphics[width=\linewidth]{figures/walsh2_dd.pdf}
    \caption{Decision tree}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.47\linewidth}
    \centering
    \includegraphics[scale=0.4]{figures/walsh2_bdd_new.pdf}
    \caption{BDD}
    \end{subfigure}
    \caption{
    Two representations of Hadamard matrix $H_4$ with the interleaved-variable ordering $\langle x_0, y_0, x_1, y_1 \rangle$.
    }
    \label{Fi:walsh2_dd_bdd}
\end{figure}



\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.5]{PatentApplication/figures/cropped-walsh2.eps.pdf}
    \caption{CFLOBDD Representation}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.5]{figures/walsh2_path.pdf}
    \caption{Path $[x_0 \mapsto F, y_0 \mapsto T, x_1 \mapsto F, y_1 \mapsto T]$}
    \end{subfigure}
    \caption{(a) The CFLOBDD representation of Hadamard matrix $H_4$ with the interleaved-variable ordering $\langle x_0, y_0, x_1,y_1 \rangle$.
    (b) The path for the assignment $[x_0 \mapsto F, y_0 \mapsto T, x_1 \mapsto F, y_1 \mapsto T]$.}
    \label{Fi:walsh2}
\end{figure}

\subsection{Encoding $H_4$ with a CFLOBDD}

Now consider the next matrix in the family of Hadamard matrices: $H_4 = H_2 \tensor H_2$.
A representation of $H_4$ requires four Boolean variables to index the matrix's elements: $x_0$ and $x_1$ form the row index, and $y_0$ and $y_1$ form the column index.
Our convention will be that $x_0$ and $y_0$ are the most-significant bit of the row and column indexes, respectively.

\figref{walsh2_dd_bdd}(a) shows the decision tree for $H_4$, which has $4$ plies and $15$ nodes.
The BDD representation of $H_4$ is shown in~\figref{walsh2_dd_bdd}(b).
Both the decision tree and the BDD use the interleaved-variable ordering: $\langle x_0,y_0,x_1,y_1 \rangle$.
With this variable ordering, the BDD requires 8 nodes.
The respective paths for the assignment $[{x_0} \mapsto F, {y_0} \mapsto T, {x_1} \mapsto F, {y_1} \mapsto T]$, which corresponds to $H_4[0,3]$, are shown in bold in \figref{walsh2_dd_bdd}(a) and \figref{walsh2_dd_bdd}(b)
(The path in the BDD only shows $x_0 \mapsto F, x_1 \mapsto F$ because the plies for $y_0$ when $x_0 \mapsto F$ and $y_1$ when $x_0 \mapsto F, x_1 \mapsto F$ are skipped).
In both cases, one starts from the top node of the structure and follows the successive ``decisions'' $F$, $T$, $F$, and $T$ to reach the terminal $1$.



Let us now see how to evaluate the assignment $[{x_0} \mapsto F, {y_0} \mapsto T, {x_1} \mapsto F, {y_1} \mapsto T]$---which corresponds to $H_4[0,3]$---by following the path highlighted in bold in~\figref{walsh2}(b).
The path starts from the level-$2$ grouping's entry vertex.
It goes to the level-$1$ grouping's entry vertex and then the fork grouping at level-$0$, where the decision for the first variable, $x_0$, is made.
Because $x_0$ has the value $F$ in the assignment, the path follows the left branch, and then returns to the level-$1$ grouping's leftmost middle vertex.
The path proceeds to the don't-care grouping at level-$0$, where the next decision---$y_0 \mapsto T$---causes it to follow the right branch and then return to the leftmost exit vertex of the level-$1$ grouping.
The path then returns to the leftmost middle vertex of the level-$2$ grouping, which leads back to the entry vertex of the level-$1$ grouping via the dashed-dotted B-connection.
The path then follows the i/dentical track as before---this time for $[{x_1} \mapsto F, {y_1} \mapsto T]$---until it again reaches the leftmost exit vertex of the level-$1$ grouping.
This time the path follows the matching dashed-dotted return edge to the leftmost exit vertex of the level-$2$ grouping, and then reaches the terminal value $1$:
i.e., $H_4[0,3]$ is $1$.



\subsection{Reuse of Groupings and Compression of Boolean Functions}
\label{Se:ReuseOfGroupings}

The reason CFLOBDDs can represent certain Boolean functions in a highly compressed fashion is the reuse of groupings that the matched-path principle enables.
As the number of Boolean variables increases, the best-case characteristics of decision trees and CFLOBDDs grow as follows:

\medskip
\noindent
\begin{minipage}{\textwidth}
\centering
  \begin{tabular}{c@{\hspace{2.0ex}}c@{\hspace{1.0ex}}|c@{\hspace{2.0ex}}c@{\hspace{1.0ex}}|@{\hspace{1.0ex}}c@{\hspace{2.0ex}}c@{\hspace{2.0ex}}c@{\hspace{2.0ex}}c}
    Boolean & Number    & \multicolumn{2}{c|@{\hspace{1.0ex}}}{Decision trees} & \multicolumn{4}{c}{CFLOBDDs (best case)} \\
    \cline{3-8}
    vars.   & of paths  & height & size      & height\footnote{The height of a CFLOBDD is the level of the outermost grouping.} & \#groupings & \#vertices & \#edges \\
    \hline
    1       & 2         & 1      & 2         & 0      & 1 & 2 & 2 \\
    2       & 4         & 2      & 4         & 1      & 2 & 5 & 6 \\
    4       & 16        & 4      & 16        & 2      & 3 & 8 & 10 \\
    8       & 256       & 8      & 256       & 3      & 4 & 11 & 14 \\
    \vdots  & \vdots    & \vdots & \vdots    & \vdots & \vdots & \vdots & \vdots \\
    $2^L$   & $2^{2^L}$ & $2^L$  & $2^{2^L}$ & $L-1$  & $L$ & $3L + 2$ & $4L + 2$ \\
    \hline
  \end{tabular}
\end{minipage}

\medskip
\noindent
The best-case CFLOBDD size (whether measured in the number of groupings, vertices, or edges) grows linearly with the level of the outermost grouping, which is \emph{logarithmic} in the number of Boolean variables.
In contrast, decision trees grow \emph{exponentially} in the number of Boolean variables.

The keys to the power that CFLOBDDs have to compress a family of Boolean functions
are two-fold:
\begin{itemize}
  \item
    The number of paths in a CFLOBDD is \emph{squared} with each increase in level by 1.\footnote{
      In a grouping at level $i$, each path through the A-connection's level-$(i\textrm{--}1)$ grouping reaches a middle vertex, where it is routed through the level-$(i\textrm{--}1)$ grouping of the vertex's $B$-connection.
      Arguing inductively, each level-$(i\textrm{--}1)$ grouping encompasses $2^{i-1}$ variables and has $2^{2^{i-1}}$ paths;
      therefore, each level-$i$ grouping encompasses $2^{i-1} + 2^{i-1} = 2 * 2^{i-1} = 2^i$ variables and has $2^{2^{i-1}} * 2^{2^{i-1}} = 2^{({2^{i-1}} +\, {2^{i-1}})} = 2^{2* {2^{i-1}}} = 2^{2^i}$ paths.
      (The base case is that each of the two possible level-$0$ groupings encompasses $1 = 2^0$ variables and has $2 = 2^{2^0}$ paths.)
    }
  \item
    The matched-path principle enables lower-level groupings to be reused via ``procedure calls.''
\end{itemize}
\twrchanged{
Consider a family of functions $F = \{ f_j \mid j \geq 0 \}$, where the $j^{\textit{th}}$ member has $2^j$ Boolean-valued arguments.
The following properties are a sufficient condition for the size of the CFLOBDDs for members of $F$ to grow linearly in the level $i$
(and therefore exhibit asymptotic best-case behavior):
\begin{enumerate}
  \item
    \label{It:ConstantSizeGrouping}
    the number of vertices in the level-$(i\textrm{+}1)$ grouping of $f_{i+1}$ is constant
  \item
    \label{It:ConstantNumberOfCalls}
    the level-$(i\textrm{+}1)$ grouping of $f_{i+1}$ makes ``procedure calls'' only to (i) the level-$i$ grouping used in the CFLOBDD for $f_i$, and (ii) the level-$i$ grouping used in the CFLOBDD for a function $g_i$, where the family of functions $G = \{ g_j \mid j \geq 0 \}$ grows linearly in the level $i$.
\end{enumerate}
}
(Here ``constant'' means ``independent of $i$.'')
In such a case, the CFLOBDD for each $f_i$ is double-exponentially smaller than the decision tree for $f_i$---i.e., of size $O(i)$ rather than $O(2^{2^i})$.
Moreover, in all such cases that we have encountered, it is possible to give an explicit algorithm for constructing the $i^{\textit{th}}$ member of $F$ that runs in time $O(i)$ and uses at most $O(i)$ space.

Properties (\ref{It:ConstantSizeGrouping}) and (\ref{It:ConstantNumberOfCalls}) can be illustrated using the family of Hadamard matrices $\{ H_{2^i} \mid i \geq 1 \}$, where $H_{2^{j+1}} = H_{2^j} \tensor H_{2^j}$ for $j \geq 1$.
First, consider the second matrix in the family: $H_4 = H_2 \tensor H_2$.
A representation of $H_4$ requires four Boolean variables to index the matrix's elements: $x_0$ and $x_1$ form the row index, and $y_0$ and $y_1$ form the column index.
Our convention will be that $x_0$ and $y_0$ are the most-significant bit of the row and column indexes, respectively.

\begin{figure}[tb!]
    \centering
    \includegraphics[height=3.5in]{figures/walsh2_expand.pdf}
    \caption{CFLOBDD for $H_4$---with the interleaved-variable ordering $\langle x_0, y_0, x_1,y_1 \rangle$---in fully expanded form.
    }
    \label{Fi:walsh2_expand}
\end{figure}

The CFLOBDD for $H_4$ has $4$ Boolean variables, and hence has $3$ levels: $0$, $1$, and $2$.
\figref{walsh2_expand} shows the ``fully-expanded form'' of the CFLOBDD that represents $H_4$.
(Following up on our procedure-call analogy, the fully-expanded form is what one obtains by cloning ``procedures'' (groupings) so that each copy of each ``procedure'' is called from exactly one place.)
The CFLOBDD in \figref{walsh2_expand} has groupings at three levels:
level $2$---the large oval labeled $L_2$;
level $1$---the three medium-sized ovals, such as $L_1$; and
level $0$---six fork-groupings and three don't-care groupings.
One can see that the same level-$1$ structures (and the level-$0$ structures that they ``call'') appears three times;
it is ``called'' once as $L_2$'s A-connection (for variables $\langle x_0, y_0 \rangle$) and twice as $L_2$'s B-connections (for variables $\langle x_1, y_1 \rangle$).
Note that the return edges from the leftmost B-connection of $L_2$ and the rightmost B-connection of $L_2$ are connected to $L_2$'s exit vertices in opposite orders: $[1,2]$ and $[2,1]$, respectively.

\begin{figure}[tb!]
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.5]{figures/walsh2_path.pdf}
    \caption{The CFLOBDD representation of Hadamard matrix $H_4$ with the interleaved-variable ordering $\langle x_0, y_0, x_1,y_1 \rangle$.
    The \textbf{bold} arrows and arcs highlight the matched path for the assignment $[x_0 \mapsto F, y_0 \mapsto T, x_1 \mapsto F, y_1 \mapsto T]$, which corresponds to $H_4[0,3]$ (with value $1$).}
    \label{Fi:walsh4_0_3_path}
    \end{subfigure}
    \quad
    \begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.5]{figures/walshK.pdf}
    \caption{Diagram of the pattern of A-connection, B-connection, and return    edges in the outermost grouping.
    }
    \label{Fi:walshKGeneralCase}
    \end{subfigure}
    \caption{Diagrams supporting the inductive argument that, with the interleaved-variable ordering, the matrices $\{ H_{2^i} \mid i \geq 1 \}$ can be constructed by successively cloning the outermost grouping:
    the level-$(i\textrm{+}1)$ grouping (i) uses the same pattern of A-connection, B-connections, and return edges found in the level-$i$ grouping, and (ii) makes just two ``calls'' on the level-$i$ grouping.
    }
    \label{Fi:walshK}
\end{figure}

The actual CFLOBDD for $H_4$, shown in \figref{walsh4_0_3_path}, makes use these commonalities to reuse instances of groupings---making ``calls'' to the same procedure---thereby reducing the size of the representation to
two level-$0$ groupings, a single level-$1$ grouping, and the level-$2$ grouping.

Now consider \figref{walshKGeneralCase}, which shows how this pattern is continued to construct the CFLOBDDs for $\{ H_{2^i} \mid i \geq 1 \}$.
\begin{description}
  \item [Property (\ref{It:ConstantSizeGrouping}):]
    \figref{walshKGeneralCase} illustrates how, with the interleaved-variable ordering, the CFLOBDD for the matrix $H_{2^{i+1}}$ can be constructed by essentially cloning the level-$i$ grouping from $H_{2^i}$.
    \Omit{The level-$(i\textrm{+}1)$ grouping (i) uses the same pattern of A-connection, B-connections, and return edges found in the level-$i$ grouping, and (ii) makes just two ``calls'' on the level-$i$ grouping.}
    The size of the outermost grouping is thus constant, independent of $i$.
  \item[Property (\ref{It:ConstantNumberOfCalls}):]
    The Kronecker product in the recursive definition of the Hadamard matrices ($H_{2^{i+1}} = H_{2^i} \tensor H_{2^i}$, for $i \geq 1$) corresponds to the reuse of lower-level groupings that the matched-path principle enables.
    The value of $i$ corresponds to the level of the highest-level grouping---$H_{2^i}$ is represented by a level-$i$ grouping---and the $\tensor$ operator on the right-hand side corresponds to $H_{2^{i+1}}$'s level-$(i\textrm{+}1)$ grouping using $H_{2^i}$'s level-$i$ grouping multiple times (cf.\ the comment in \footnoteref{KroneckerProduct} that ``the recursive rule `$H_{2^{i+1}} = H_{2^i} \tensor H_{2^i}$' fits particularly well with the internal structure of CFLOBDDs'').
    \figref{walshK}(b) shows that level-$(i\textrm{+}1)$ grouping makes just two ``calls'' on the level-$i$ grouping.
\end{description}
Consequently, $H_{2^i}$ can be constructed in time $O(i)$ and space $O(i)$ (see also \sectref{HadamardMatrix} and \algref{HAlgo}).

It should be noted that no information-theoretic limit is being violated here.
Not all families of functions can be represented with CFLOBDDs in which each level has a constant number of groupings, each of constant size---and thus, not every function over Boolean-valued arguments can be represented in such a compressed fashion (i.e., logarithmic in the number of Boolean variables, or, equivalently, doubly logarithmic in the size of the decision tree).
However, the potential benefit of CFLOBDDs is that, just as with BDDs, there may turn out to be enough regularity in problems that arise in practice that CFLOBDDs stay of manageable size.
Moreover, doubly-exponential compression (or any kind of super-exponential compression) could allow problems to be completed much faster (due to the smaller-sized structures involved), or allow far larger problems to be addressed than has been possible heretofore.

For example, if you want to tackle a problem with ${2^{20}} = \textrm{1,048,576}$ Boolean variables (and thus a state space of size ${2^{2^{20}}} = {2^{\textrm{1,048,576}}} \approx {6.74 \times 10^{\textrm{315,652}}}$), it might be possible to get by with CFLOBDDs consisting of a small multiple of $\log_2 \log_2 {2^{2^{20}}} = 20$ groupings (arranged in levels $0 \textrm{-} 19$).
In contrast, a successful use of BDDs is likely to need BDDs with (small multiples of) $\textrm{1,048,576}$ nodes.
Not only would CFLOBDDs potentially save a great deal of space, but operations on CFLOBDDs could potentially be performed much faster than operations on the corresponding BDDs.

However, even this hypothetical example with $20$ levels is ``small-think.''
In \sectref{ResearchQuestionOne}, we describe how we created a CFLOBDD for an interesting relation (namely, addition) in which we used $2^{23} + 2$ $= \textrm{8,388,610}$ levels, and thus $2^{\textrm{8,388,610}}$ $\cong 1.706 \times 10^{\textrm{2,525,223}}$ Boolean variables.
Because of a slightly technical alignment issue, we deliberately wasted one-quarter of the variables;
thus, we used ``only'' $1.2795 \times 10^{\textrm{2,525,223}}$ Boolean variables.
Consequently, the size of the state space for this relation is the hard-to-comprehend number $2^{1.2795 \times 10^{\textrm{2,525,223}}}$ states.

\Omit{
Recapping the discussion in this section, in the best case, a family of Boolean functions (such as the Hadamard matrices) can be succinctly represented by a family of CFLOBDDs, each member of which exhibits a \textit{double-exponential} compression in the overall size of the structure, compared to the size of the decision tree for the function.
}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 

==> polynomial-bdd-simulation-by-cflobdds.tex <==
% -*- TeX-master: t; TeX-PDF-mode: t -*-

\section{Polynomial Simulation of BDDs by CFLOBDDs}
\label{Se:PolynomialBDDSimulation}

\twr{UNDER CONSTRUCTION}

\twrnew{
\sectref{efficient-relations} showed that there is an exponential gap between CFLOBDDs and BDDs:
the CFLOBDD for a function $f$ can be exponentially smaller than
any BDD for $f$, regardless of the variable order used in the BDD.
This section considers whether there is such a separation in the opposite direction, and answers the question in the negative:
for any Boolean function $f$ over $n = 2^k$ variables whose BDD representation using variable ordering $\pi$ is of size $S$, the CFLOBDD for $f$ that uses variable ordering $\pi$ is no larger than $n(n+1)S$.
Thus, a BDD always has an ``efficient'' simulation---in the sense of the sizes being polynomially related---via a CFLOBDD.
}

\twrnew{
To establish this result, we will demonstrate the simulation for so-called quasi-reduced BDDs (QBDDs).
\emph{Quasi-reduced BDDs} are the version of BDDs in which variable ordering is respected, but don't-care nodes are \emph{not} removed (i.e., plies are not skipped), and thus all paths from the root to a leaf have length $n$, where $n$ is the number of variables.
The size of a quasi-reduced BDD is at most a factor of $n+1$ larger than the size of the corresponding ROBDD \cite[Thm.\ 3.2.3]{Book:Wegener00}.
Because $n = 2^k$, the simulating CFLOBDD has $k$ levels, hence our goal is to show that if the QBDD representation of $g$ using variable ordering $\pi$ is of size $Q$, then the CFLOBDD for $g$ using $\pi$ is no larger than $2^k Q$.
}

\twrnew{
Elements of the construction:
\begin{itemize}
  \item
    We compare the number of nodes and edges of the QBDD to the number of vertices and edges of the CFLOBDD, but to avoid getting overburdened in details, we will not count the cost of terminal values, nor---in the case of CFLOBDDs---value edges.
    (In the case of Boolean-valued functions, there are at most two terminal values, and the CFLOBDD has at most two value edges.)
  \item
    We give an inductive argument.
    However, when a level-$k$ CFLOBDD is decomposed into its constituent level-$k\textbf{-}1$ A-connection and B-connection proto-CFLOBDDs, the later form a \emph{forest} of shared objects, where the entry points to the forest are the entry vertices of the level-$k\textbf{-}1$ proto-CFLOBDDs.
    Similarly, we will consider a collection of ``half-height'' fragments of QBDDs, which form their own forest of shared objects.
    Thus, to establish the desired result by induction, we must prove a more general property---namely, that a shared \emph{forest} of QBDDs of height-$2^k$ can be simulated by a shared forest of level-$k$ CFLOBDDs that is larger by at most a factor of $2^k$.
\end{itemize}
}


==> tmp.tex <==
%% Temporary text

\subsection{CFLOBDDs}
\label{Se:CFLOBDDs}

CFLOBDDs~\cite{reps2002method}---Context-Free-Language Ordered Binary
Decision Diagrams---are a data structure that stores data in a highly
compressed fashion.
As a representation of a decision tree over a set of Boolean-valued
decision variables, a CFLOBDD can provide a \emph{double-exponential
compression} in space over the decision tree.
When a decision tree $T$ is represented using an OBDD (Ordered Binary
Decision Diagram) or a MTBDD (Multi-Terminal Binary Decision Diagram),
it can provide only an \emph{exponential compression in space} over $T$;
thus, CFLOBDDs can sometimes provide an additional exponential degree
of compression over OBDDs/MTBDDs.
Similar to OBDDs/MTBDDs, CFLOBDDs can represent functions, matrices,
graphs, relations, etc.\ (using either binary-valued terminals or
multi-valued terminals, as appropriate), again with the possible
advantage of an additional exponential degree of compression over
OBDDs/MTBDDs.
Even for objects that do not fall into the best-case scenario of
perfect double-exponential compression, CFLOBDDs may provide better
compression than OBDDs and MTBDDs.

\begin{figure*}
\centering
\begin{tabular}{c@{\hspace{.1in}}c@{\hspace{.1in}}c}
        \includegraphics[height=1.0in]{figures/proto3Tree.eps}
     &  \includegraphics[height=2.0in]{figures/proto3Expanded.eps}
     &  \includegraphics[height=2.0in]{figures/proto3.eps}
    \\  (a) Decision tree for a function of
     &  (b) Fully expanded form
     &  (c) Multi-terminal CFLOBDD
    \\      type Bool $\times$ Bool $\rightarrow$ $\{a,b,c\}$
     &  
     &      for decision-tree (a)
\end{tabular}
\caption{}
\label{Fi:MultiTerminal}
\end{figure*}

A BDD can be considered as a folding of a decision tree, forming a DAG, leading to \emph{exponential compression}.
A CFLOBDD can be taken as a further folding of a BDD, giving a \emph{double-exponential compression}, thereby forming a cyclic graph.
\figref{MultiTerminal} shows multi-terminal CFLOBDD. Similar to Boolean-valued BDDs and Multi-Terminal BDDs, CFLOBDDs can have boolean terminals or multi-valued terminals.
We will refer to both of them as CFLOBDDs and the type of the terminals will be understood based on the context.
The CFLOBDDs have different structural components as described below:
\begin{itemize}
\item The vertices are grouped by circles/ovals into \emph{levels}. 
The smaller ones represent \emph{level-0} groupings and every subsequent grouping represents one level higher (\emph{level-1}, \emph{level-2} and so on).
\item The vertex at the top of a grouping is called \emph{entry vertex}, the vertices at the middle of the grouping are called \emph{middle vertices} 
and the vertices at the bottom of the grouping are called \emph{exit vertices}. We assume that the middle vertices and the exit vertices are arranged in a fixed known order.
\item The edge that emerges from the entry vertex of a grouping $g$ of level $i$ and lead to a grouping of level $i-1$ is called $g$'s \emph{A-connection}.
\item The edges that emerge from any of the middle vertices of grouping $g$ at level $i$ and lead to a grouping of level $i-1$ are called $g$'s \emph{B-connections}.
\item \emph{Return Edges} of grouping $g$ at level $i$ are the edges that emerge from the exit vertices of a grouping of level $i-1$ and lead to one of the exit vertices of $g$.
\item The edges from exit vertices of the highest grouping of the CFLOBDD that lead to values - either boolean-valued or multi-valued - are termed as \emph{value edges}.
In case of Boolean-valued CFLOBDD, there would be at most two exit vertices and two value edges uniquely mapped to \{F,T\}.
In case of multi-terminal CFLOBDD, there could be arbitrary number of exit vertices and value edges, uniquely mapped to a set of values.
\item All the decisions are taken at the entry vertex of \emph{level-0} grouping, that is, they \emph{level-0} groupings correspond to a decision in the corresponding decision tree.
The decisions at \emph{level-0} are of two types:
\begin{itemize}
\item If the decisions depend on the decision variables corresponding to this \emph{level-0} grouping, then it is called \emph{fork grouping}.
\item In case, the decisions do not depend on this $level-0$ grouping variables, then it is called \emph{don't-care grouping}.
\end{itemize}
\end{itemize}
Every path in a decision tree can be found in its corresponding CFLOBDD. Given a path formed by "decisions" at every decision variable in decision tree,
a similar path can be formed from the entry vertex of the highest-level grouping with "decisions" for every decision variable in the same sequence every time a $level-0$ is encountered.
Therefore, a CFLOBDD that represents every path of a decision tree has a compressed representation compared to the latter. 
This is mainly due to the utilization of the same groupings at different parts of the data structure, similar to procedure calls.

To illustrate how CFLOBDDs are similar to procedure calls, consider a simple program with five functions $f_a$, $f_b$, $f_c$, $f_d$ and $f_e$ with the following conditions:
\begin{itemize}
\item $f_a$ calls $f_b$ and $f_d$.
\item $f_e$ calls $f_b$ and $f_d$.
\item $f_b$ calls $f_c$.
\item $f_d$ calls $f_c$.
\item $f_c$ does not call any function.
\end{itemize}

Every oval/circle in \figref{callgraph} corresponds to a function. The figure shows the call graph of the program. 
For every call arc $f_i$ to $f_j$, there is a corresponding return arc $f_j$ to $f_i$.
We can observe that every function is represented only once, however every call to the function in the program is represented by an incoming (call arcs) and outgoing edges (return arcs).
Every pair of incoming and outgoing edges is called a \emph{matched path}.
The matched path principle of procedure calls is used in CFLOBDDs which helps in \emph{double-exponential compression in space}.

\begin{figure*}
  \centering
  \includegraphics[scale=0.5]{newFigures/callgraph.eps}
  \caption{Call graph}
  \label{Fi:callgraph}
\end{figure*}

\iffalse
\twr{MISSING/NEEDS CLARIFICATION:
Explanations for many of the items can be taken from the patent application.
\begin{itemize}
  \item
    Describe the structural elements of a CFLOBDD: \emph{grouping}, \emph{level}, decision variables
    modeled only at level 0 (\emph{fork grouping} versus \emph{no-distinction grouping}, and 
    the $A$-connection and $B$-connections.
  \item
    Quasi-reduced BDDs have no transformation to introduce variable skipping when the BDD
    has a ``don't-care'' node.
    That is, in an ROBDD, when a node $n_1$ has two child pointers
    that point to the same node $n_2$, $n_1$ is removed, and all child pointers that point to
    $n_1$ are redirected to $n_2$;
    In a quasi-reduced BDD, $n_1$ is kept in the data structure.
    Thus, each root-to-leaf path in a quasi-reduced BDD visits a node for each of the decision variables
    (in the global variable-ordering sequence) $x_0, x_1, \ldots, x_{n-1}$.
    Similarly, CFLOBDDs have no operation to remove ``redundant'' decisions, and
    each root-to-leaf path in a CFLOBDD visits a level-0 grouping for each of the
    decision variables (in the global variable-ordering sequence).
    \hspace*{1.5ex}
    Henceforth, whenever we refer to a ``BDD'' we mean a ``quasi-reduced BDD.''
  \item
    A CFLOBDD is like a BDD with procedure calls.
    In particular, explain the procedure-call nature of the $A$-connection and the $B$-connections.
  \item
    Illustrate: A decision tree represented as a tree, a BDD, and a CFLOBDD.
  \item
    Multi-terminal CFLOBDDs: EXPLAIN.
    We refer to both Boolean CFLOBDDs and multi-terminal CFLOBDDs as ``CFLOBDDs;''
    which kind of object is intended should be clear from context.
  \item
    Give a brief explanation of Boolean operations on CFLOBDDs:
    as with Boolean BDDs and MTBDDs, a binary operation
    (i) performs a ``product'' construction;
    (ii) applies the appropriate operation on each the pair of elements at the leaf; and
    (iii) performs a reduction step induced by which leaves have the same value.
    Step (iii) is somewhat more involved for CFLOBDDs than the corresponding reduction step
    for BDDs.
\end{itemize}
}
\fi
\begin{table}[!ht]
\centering
\caption{Growth of CFLOBDD}
\label{Ta:growth-cflobdd}
\begin{tabular}{|c|c|c|}
\hline
Max.\ Level & No.\ of Boolean Variables & Number of Paths (Decision-Tree Leaves)\\
\hline
0 & 1 & 2\\
\hline
1 & 2 & 4\\
\hline
2 & 4 & 16\\
\hline
3 & 8 & 256\\
\hline
\vdots & \vdots & \vdots\\
\hline
k & $2^k$ & $2^{2^k}$\\
\hline
\end{tabular}
\end{table}

\tableref{growth-cflobdd} shows the growth of CFLOBDD as the number of
decision/Boolean variables increase.
Hence, given $k$ outcomes for $\log{}(k)$ decision variables, the size of CFLOBDD is
$\log{}(\log{}(k))$ in the best case, whereas in the case of BDDs, the
size would be $\log{}k$---i.e., equal to number of decision variables in the
best case.
With BDDs, only about 300 decision variables can be used in practice
but with CFLOBDDs, 512 variables can be represented only with 9
levels.
%\twr{Explain how the procedure-call nature of the $A$-connection and the $B$-connections
%is responsible for the double-exponential compression in space.}

\subsection{Representing Matrices and Vectors Using CFLOBDDs}
\label{Se:RepresentingMatricesAndVectorsUsingCFLOBDDs}

As one does with decision trees and BDDs, to represent matrices or vectors
with a CFLOBDD, we partition the Boolean decision variables into two groups;
their values represent the respective bits of the two indices of a given matrix
element.
Every path in the CFLOBDD (or decision tree or BDD) leads to an entry of
the matrix or vector.

\paragraph{CFLOBDD Represention of Matrix:}
We call each of the two groups of decision variables a \emph{vocabulary}.
We represent a matrix with two vocabularies---one for the row index and another for
column index.
Consider $(X, Y) = (\Pair{x_0}{x_1, \hdots, x_n},\Pair{y_0}{y_1,
\hdots, y_n})$, where $X$, $Y$ are the vocabularies, $x_i$, $y_i$ ,
$\forall i\in [0\hdots n]$, are the decision variables corresponding
to each of the vocabularies and $n = \log_2 {(\emph{number of
rows/columns})}$.
The $2n$ boolean variables are used to represent a matrix $M$ of size $2^n \times 2^n$.
The variables of vocabulary $X$ correspond to each successive bits of row indices and
that of $Y$ represent successive bits of column indices.
We interleave the decision variables of the two vocabularies when representing
the matrix as a BDD/CFLOBDD.
~\figrefs{CFLOBDDRepeSampleMatrix1}{CFLOBDDRepeSampleMatrix2} show the CFLOBDD and BDD
representations of two sample matrices.
Both the matrices use two
interleaved vocabularies - $(\langle{x_0\rangle},\langle{y_0\rangle})$
and $(\Pair{x_0}{x_1},\Pair{y_0}{y_1})$ respectively, for
representation.

Every grouping at level $i$ of a CFLOBDD can be (roughly) viewed as a kronecker product 
of the matrix represented by the grouping at level $i-1$ through \emph{A connection} and the matrix represented by the grouping at level $i-1$ through \emph{B connection}. If $(x_0, y_0, \hdots, x_n, y_n)$ represent matrix $X$ (of grouping at \emph{A connection}) and $(z_0, w_0, \hdots, z_n, w_n)$ represent matrix $Y$ (of grouping at \emph{B connection}), then the kronecker product $X \tensor Y$ is represented by the concatenation of the variables to form $(x_0, y_0, \hdots, x_n, y_n, z_0, w_0, \hdots, z_n, w_n)$ (grouping at level $i$).

Consider the following matrices A, B and their kronecker product:
\[
  A = \kbordermatrix{
            & 00 & 01 \\
          00 & 1 & 1 \\
          01 & 1 & 1
      }
\]

\[
  B = \kbordermatrix{
            & 00 & 01 \\
          00 & 1 & 1 \\
          01 & 0 & 0
      }
\]

\[
  A \tensor B = \kbordermatrix{
                  & 00 & 01 \\
                  00 & 1 \cdot B & 1 \cdot B\\
                  01 & 1 \cdot B & 1 \cdot B
                }
\]

\[
  A \tensor B = \kbordermatrix{
                    & 00 & 01 & 10 & 11 \\
                  00 &  1 & 1 & 1 & 1 \\
                  01 &  0 & 0 & 0 & 0 \\
                  10 &  1 & 1 & 1 & 1 \\
                  11 &  0 & 0 & 0 & 0
                }
\]

\begin{figure*}[!ht]
\centering
\begin{tabular}{c@{\hspace{.25in}}c@{\hspace{.25in}}c}
    \includegraphics[height=2.5in]{newFigures/AMatrix.eps}
  & \includegraphics[height=2.5in]{newFigures/BMatrix.eps}
 \\
    (a) Matrix $A$
  & (b) Matrix $B$
\end{tabular}
\end{figure*}

\begin{figure*}[!ht]
  \centering
  \includegraphics[scale=0.5]{newFigures/ATensorB.eps}
  \caption{Matrix $A \tensor B$}
\end{figure*}

The figures show the CFLOBDDs represented by matrices $A$ and $B$ and $A \tensor B$. We can observe that the nature of $A connection$ and $B connection$ in CFLOBDD is similar to the kronecker product of matrices $A$ and $B$.

Note that the CFLOBDD representing the kronecker product uses 2 vocabularies. 
We can create CFLOBDDs representing the kronecker product of the same vertices with 4 vocabularies 
where the decision variables of the base matrices are \emph{interleaved} and not concatenated.
Hence, in such cases, $(x_0, y_0,, z_0, w_0, \hdots, x_n, y_n, z_n, w_n)$ represent the ordering of
the variables representing the CFLOBDD. We will show the use of this approach in \sectref{CFLOBDDRep}.

\begin{figure*}[!ht]
\begin{center}
\includegraphics[scale=0.75]{newFigures/CFLOBDD-1.eps}
\end{center}
\caption{CFLOBDD and BDD representations of a sample matrix (2 variables).
  %\twr{(i) Need to add labels in $\{ 0,1 \}$ to the matrix, each ply of the BDD, and the level-0 node of the CFLOBDD;
  %     (ii) Probably better to use the Hadamard matrix, to show two terminals, 1 and $-1$
  %    }
}
\label{Fi:CFLOBDDRepeSampleMatrix1}
\end{figure*}
\begin{figure*}[!ht]
\begin{center}
\includegraphics[scale=0.5]{newFigures/CFLOBDD-2.eps}
\end{center}
\caption{CFLOBDD and BDD representations of a sample matrix (4 variables)}
\label{Fi:CFLOBDDRepeSampleMatrix2}
\end{figure*}

%\twr{Explain how the procedure-call nature of the $A$-connection and the $B$-connections in a CFLOBDD
%correspond to a Kronecker product of the $A$-connection and the $B$-connections (roughly).
%Illustrate an easy case of the Kronecker product of two matrices.
%}

\paragraph{CFLOBDD Representation of a Vector:}
We represent a vector using one vocabulary, i.e., one set of decision variables for the row index.
Consider the vector $X = \B{x_0, x_1, \ldots, x_n}^t$, as the decision variables corresponding to the row indices. Note that, similar to matrices, $n = \log{(\textit{number of rows})}$.
~\figrefs{CFLOBDDRepeSampleVector1}{CFLOBDDRepeSampleVector2} show the CFLOBDD and ROBDD representations of two sample vectors. The vectors use one decision variable - $\langle{x_0 \rangle}$ and two decision variables - $\Pair{x_0}{x_1}$ respectively, for representation.

\begin{figure*}[!ht]
  \centering
  \includegraphics[scale=0.75]{newFigures/CFLOBDD-3.eps}
  \caption{CFLOBDD and BDD representations of a sample vector (1 variable)}
  \label{Fi:CFLOBDDRepeSampleVector1}
\end{figure*}

\begin{figure*}[!ht]
  \centering
  \includegraphics[scale=0.5]{newFigures/CFLOBDD-4.eps}
  \caption{CFLOBDD and BDD representations of a sample vector (2 variables)}
  \label{Fi:CFLOBDDRepeSampleVector2}
\end{figure*}

\subsection{Linear Solver using Howell Matrices}
\label{Se:LinearSolverUsingHowellMatrices}

After sampling/measuring the output of final vector $b$, the obtained $x$ part of the sampled bits are used to solve for hidden vector $s$.
We obtain $(n-1)$ non-zero vectors ($n$ vectors including the zero vector) which are used as constraints to obtain $s$.
We use dualization of Howell matrices to solve for the hidden vector $s$.
Let $x_0 = \vec{0}, x_1, \hdots , x_{n-1}$ be the measured vectors such that $x_0 \cdot s = 0, \hdots x_{n-1}, \cdot s = 0$. These linear equations are added to a solver to find $s$.

We use a matrix $M$ to represent these set of linear equations. Every row of the matrix $M$ corresponds to a vector from $x_0,\hdots ,x_{n-1}$, prepended with a $0$ for the constant part which is zero. We can say that $Ms'^{\,t} = 0$, where $s'$ is the vector $s$ with an extra bit prepended.
Thus, finding the null space of $M$ gives the solution for $s$. We use howellization and dualization of matrices for finding the null space of $M$. Note that all the operations are performed in Boolean space.

Elder et al.~\cite{elder2014abstract} describe the formation of Howell matrices and the
dualization of Howell matrices. 
A matrix $\mathcal{H}$ is in Howell form if 
\begin{enumerate}
\item $\mathcal{H}$ is in row-echleon form and has all non-zero rows,
\item the leading value of every row is a power of two,
\item each leading value is the largest in its column,
\item for every row $\vec{r}$ of $\mathcal{H}$, for any $p \in \mathbb{Z}$, if $i$ is the leading index of $2^p\vec{r}$, then $2^p\vec{r} \in row([\mathcal{H}])_i$.
\end{enumerate}

The process of converting a matrix into a howell form is termed as howellization and it is similar to the standard process of Gaussian-elimination as described in ~\cite{elder2014abstract} and runs with the same cubic-time complexity as of Gaussian-elimination.
We convert the matrix $M$ into howell form, $\mathcal{H}$. We can note that the howellization of $M$ would eliminate the row corresponding to $\vec{0}$ obeying Point $1$. As every value is either 0 or 1, Point $2$ always holds. Since the space is boolean, Point $4$ is already handled in $M$. Howellization ensures that Point $3$ is also satisified in $\mathcal{H}$. After the transformation, the rows in $\mathcal{H}$ become orthogonal to each other.

For the running example, the sampled vectors are $x_0 = 00$ and $x_1 = 01$. The matrix $M$ and howell matrix $\mathcal{H}$ for the example would be
\[
M = \kbordermatrix{
     & 1 & X_0 & X_1\\
    x_0 & 0 & 0 & 0\\
    x_1 & 0 & 0 & 1
  }
\]
\[
\mathcal{H} = \kbordermatrix{
    & 1 & X_0 & X_1\\
    & 0 & 0 & 1\\
  }
\]

The notation of $1$ at the top of the matrices $M$ and $\mathcal{H}$ correspond to the constant value of the linear equations, which is $0$ for all vectors in the set of linear equations. The notation of $X_0,\hdots , X_{n-1}$ (here, $X_0, X_1$) represent the corresponding bits in each of the sampled vectors.

To solve for $s$, we need to find the null space of $\mathcal{H}$. We use the theorem by Elder et al.~\cite{elder2014abstract} that 

\[
  null^t\;\mathcal{H} = row\;Dualize(\mathcal{H})
\]

We use the dualization operations mentioned in ~\cite{elder2014abstract} to obtain the dualization of $\mathcal{H}$ -- $Dualize(\mathcal{H})$.
For the running example, $Dualize(\mathcal{H})$ would be
\[
  Dualize(\mathcal{H}) = \kbordermatrix{
                            & 1 & s_0 & s_1\\
                            & 0 & 0 & 0\\
                            & 0 & 1 & 0\\
                          }
\]

The $s_0,\hdots , s_{n-1}$ (here $s_0,s_1$) represent the bits of the vector $s$. The row space of $Dualize(\mathcal{H})$ correspond to the hidden vector of $s$. We get two solutions -- $00$ and $10$. $00$ is a trivial solution to the set of linear equations and therefore not considered. Hence, we get $s = 10$ as the hidden vector for the current example.

